SAFE-SVD: Sensitivity-Aware Fidelity-Enforcing SVD for Physics Foundation Models

We propose a new method for compressing physics foundation models (PFMs) which is a new trend in AI for Science. While model compression is essential for reducing memory use and accelerating inference in large foundation models, it remains under-explored for PFMs, where preserving physical fidelity is crucial. The challenge lies in the functional nature of physics data, where partial derivatives encode spatiotemporal dynamics and exhibit high sensitivity to compression. Conventional compression methods ignore this structure, often causing severe performance degradation or failure. To address this, we introduce a sensitivity-aware fidelity-enforcing compression framework that explicitly models loss-aware layer sensitivity in the output function space during compression. This provides a new route to compressing scientific foundation models while preserving accuracy and physical fidelity. Experiments show substantial gains over existing methods across multiple models and datasets, achieving significantly higher compression ratios while maintaining accuracy, in some cases by orders of magnitude. More broadly, the work potentially leads to a new subfield of efficient, deployable, and sustainable scientific foundation models in AI for Science.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{blue}[TODO: #1]}}
\newcommand{\HW}[1]{\textbf{\color{red}[HW: #1]}}
\newcommand{\added}[1]{\textcolor{green!60!black}{#1}}
\newcommand{\removed}[1]{\textcolor{red!70!black}{\sout{#1}}}

\RequirePackage{times}    % Integrate Times for here
\RequirePackage{xspace}
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{graphicx}
\RequirePackage{amsmath}
\RequirePackage{booktabs}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\newcommand{\mat}[1]{\mathbf{#1}}


\AtEndPreamble{
    \usepackage[capitalize]{cleveref}
    \crefname{section}{Sec.}{Secs.}
    \Crefname{section}{Section}{Sections}
    \Crefname{table}{Table}{Tables}
    \crefname{table}{Tab.}{Tabs.}
}

%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{tabularx}
\usepackage{multirow}

\usepackage{enumitem}
\setlist[itemize]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}
\setlist[enumerate]{noitemsep, topsep=2pt, parsep=0pt, partopsep=0pt}

\setlength{\textfloatsep}{12pt}
\setlength{\floatsep}{12pt}
\setlength{\intextsep}{12pt}
\setlength{\tabcolsep}{3pt}

\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{0pt}

% Define colors
\definecolor{best}{HTML}{D5E8D4} %Light Green 
\definecolor{second}{HTML}{FFF2CC} % Light Yellow 

\newcommand{\colw}{0.135\textwidth}
%\newcommand{\figrow}[2]{%
%    \textbf{#1}\par\vspace{2pt}
%    \includegraphics[width=\colw]{#2/1.png}
%    \includegraphics[width=\colw]{#2/2.png}
%    \includegraphics[width=\colw]{#2/3.png}
%    \includegraphics[width=\colw]{#2/4.png}
%    \includegraphics[width=\colw]{#2/5.png}
%    \includegraphics[width=\colw]{#2/6.png}
%    \includegraphics[width=\colw]{#2/gt.png}
%    \par\vspace{6pt}
%}

\newcommand{\figrow}[2]{%
    \textbf{#1}\par\vspace{1pt}

    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_iclr.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_iclr_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/4dgs_cvpr.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/4dgs_cvpr_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ex4dgs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ex4dgs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/ftgs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/ftgs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/ftgs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphigs.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphigs_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphigs_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/graphits.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/graphits_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/graphits_b.png}
    \end{minipage}
    \begin{minipage}{\colw}\centering
        \includegraphics[width=\linewidth]{#2/gt.png}\\[0.01\linewidth]
        \includegraphics[width=0.49\linewidth]{#2/gt_a.png}\hfill
        \includegraphics[width=0.49\linewidth]{#2/gt_b.png}
    \end{minipage}

    \par\vspace{1pt}
}

% ===== SPLIT LAYOUT (4 items top, 3 items bottom) =====
\newcommand{\figrowSplit}[1]{%

  \def\sw{0.24\linewidth}%
  
  % --- ROW 1: Competitors (4 items) ---
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-1 \cite{yang2023gs4d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_iclr.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_iclr_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize 4DGS-2 \cite{wu20244d}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/4dgs_cvpr.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/4dgs_cvpr_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize Ex4DGS \cite{lee2024fully}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ex4dgs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ex4dgs_b.png}
  \end{minipage}\hfill
  \begin{minipage}[t]{\sw}\centering\scriptsize FTGS \cite{wang2025freetimegs}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/ftgs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/ftgs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/ftgs_b.png}
  \end{minipage}
  
  \par\vspace{6pt} % Gap between top and bottom rows
  
  % --- ROW 2: Ours + GT (3 items, Centered) ---
  {\centering
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiGS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphigs.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphigs_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphigs_b.png}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize \textbf{Ours (GraphiTS)}\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/graphits.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/graphits_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/graphits_b.png}
  \end{minipage}\hspace{2mm} % Slight gap
  \begin{minipage}[t]{\sw}\centering\scriptsize GT\par\vspace{1pt}
    \includegraphics[width=\linewidth]{#1/gt.png}\\[0.01\linewidth]
    \includegraphics[width=0.49\linewidth]{#1/gt_a.png}\hfill
    \includegraphics[width=0.49\linewidth]{#1/gt_b.png}
  \end{minipage}
  \par}
}

\newcommand{\figrowCrops}[1]{%
  % Configuration
  \setlength{\tabcolsep}{1pt} % Minimal horizontal gap
  \renewcommand{\arraystretch}{0.5} % Minimal vertical gap
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    \begin{tabular}{@{}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      % Note: I used \parbox on the left label, so these will align nicely
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Width 0.163 fills the 6-column space perfectly (6 * 0.163 ~ 0.98)
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_a.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_a.png} \\[1pt]

      % --- Row 2: Crop B ---
      \includegraphics[width=0.163\linewidth]{#1/4dgs_iclr_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/4dgs_cvpr_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/ex4dgs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/ftgs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphigs_b.png} &
      \includegraphics[width=0.163\linewidth]{#1/graphits_b.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWL}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth (Unchanged) ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    % Label in 2 lines to match the height of headers on the right
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: 1 label column + 6 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row: Method Names ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/4dgs_iclr_#2_a.png} &
      \vcimg{#1/4dgs_cvpr_#2_a.png} &
      \vcimg{#1/ex4dgs_#2_a.png} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/graphigs_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#3_a.png} &
      \vcimg{#1/4dgs_cvpr_#3_a.png} &
      \vcimg{#1/ex4dgs_#3_a.png} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/graphigs_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsThreeRowWL}[7]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Wraps image in a box aligned at its vertical center
  \def\vcimg##1{\parbox[c]{0.153\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  % Wraps label in a box aligned at its vertical center
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 6 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 7 columns: Label + 1pt Gap + Method + 1pt Gap + Method ...
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      &
      \parbox{1.6cm}{\centering 4DGS-1\\\cite{yang2023gs4d}} & 
      \parbox{1.6cm}{\centering 4DGS-2\\\cite{wu20244d}} & 
      \parbox{1.6cm}{\centering Ex4DGS\\\cite{lee2024fully}} & 
      \parbox{1.6cm}{\centering FTGS\\\cite{wang2025freetimegs}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiGS}\\\textbf{(Ours)}} & 
      \parbox{1.6cm}{\centering \textbf{GraphiTS}\\\textbf{(Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#5} &
      \vcimg{#1/4dgs_iclr_#2_a.png} &
      \vcimg{#1/4dgs_cvpr_#2_a.png} &
      \vcimg{#1/ex4dgs_#2_a.png} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/graphigs_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#6} &
      \vcimg{#1/4dgs_iclr_#3_a.png} &
      \vcimg{#1/4dgs_cvpr_#3_a.png} &
      \vcimg{#1/ex4dgs_#3_a.png} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/graphigs_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 3: Crop C ---
      \vclbl{#7} &
      \vcimg{#1/4dgs_iclr_#4_a.png} &
      \vcimg{#1/4dgs_cvpr_#4_a.png} &
      \vcimg{#1/ex4dgs_#4_a.png} &
      \vcimg{#1/ftgs_#4_a.png} &
      \vcimg{#1/graphigs_#4_a.png} &
      \vcimg{#1/graphits_#4_a.png} \\
      
    \end{tabular}
  \end{minipage}
}

\newcommand{\figrowCropsTwoRowWLShort}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} & 
      \parbox{2.5cm}{\centering W/O Upgrade} & 
      \parbox{2.5cm}{\centering W Upgrade} \\[5pt]
      
      % --- Row 1: Crop A ---
      % Uses #2 for filename suffix, #4 for Label
      \vclbl{#4} &
      \vcimg{#1/ftgs_#2_a.png} &
      \vcimg{#1/upgrade_#2_a.png} &
      \vcimg{#1/ftgs_#2_b.png} &
      \vcimg{#1/upgrade_#2_b.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      % Uses #3 for filename suffix, #5 for Label
      \vclbl{#5} &
      \vcimg{#1/ftgs_#3_a.png} &
      \vcimg{#1/upgrade_#3_a.png} &
      \vcimg{#1/ftgs_#3_b.png} &
      \vcimg{#1/upgrade_#3_b.png} \\
      
    \end{tabular}
  \end{minipage}
}

% \newcommand{\figrowCropsTwoRowWLShortAbl_old}[5]{%
%   % Configuration
%   \setlength{\tabcolsep}{0pt} 
%   \renewcommand{\arraystretch}{0.5} 
  
%   % --- Internal Helpers for Vertical Centering ---
%   % Grid images set to 0.30 to represent ~30% of the RIGHT block (making them small)
%   \def\vcimg##1{\parbox[c]{0.30\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
%   \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
%   % --- CENTERING WRAPPER ---
%   \centering
  
%   % --- Left Block: Ground Truth (Restored to Large Size) ---
%   \begin{minipage}[c]{0.28\linewidth} 
%     \centering
%     \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
%     \includegraphics[width=\linewidth]{#1/gt.png}
%   \end{minipage}%
%   \hspace{4pt}% Small fixed gap
%   % --- Right Block: 3 Methods (Constrained Width) ---
%   \begin{minipage}[c]{0.60\linewidth}
%     \centering
%     \tiny 
%     \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{\hspace{2pt}}c@{}}
%       % --- Header Row ---
%       % Headers match the image width (0.30)
%       &
%       \parbox{0.30\linewidth}{\centering W/O Higher Order Dynamics} & 
%       \parbox{0.30\linewidth}{\centering W/O $P(\alpha \mid \theta, C, T)$} & 
%       \parbox{0.30\linewidth}{\centering \textbf{GraphiTS (Ours)}} \\[5pt]
      
%       % --- Row 1: Crop A ---
%       \vclbl{#4} &
%       \vcimg{#1/no_higher_#2_a.png} &
%       \vcimg{#1/no_likeli_#2_a.png} &
%       \vcimg{#1/graphits_#2_a.png} \\
%       \noalign{\vspace{1pt}} 

%       % --- Row 2: Crop B ---
%       \vclbl{#5} &
%       \vcimg{#1/no_higher_#3_a.png} &
%       \vcimg{#1/no_likeli_#3_a.png} &
%       \vcimg{#1/graphits_#3_a.png} \\
      
%     \end{tabular}
%   \end{minipage}
% }

\newcommand{\figrowCropsTwoRowWLShortAbl}[5]{%
  % Configuration
  \setlength{\tabcolsep}{0pt} % We control spacing manually with @{\hspace{...}}
  \renewcommand{\arraystretch}{0.5} % Keep text tight
  
  % --- Internal Helpers for Vertical Centering ---
  % Increased width to 0.235 to fill space with only 4 images
  \def\vcimg##1{\parbox[c]{0.21\linewidth}{\includegraphics[width=\linewidth]{##1}}}%
  \def\vclbl##1{\parbox[c]{1em}{\centering\rotatebox{90}{\scriptsize \textbf{##1}}}}%
  
  % --- Left Block: Full Ground Truth ---
  \begin{minipage}[c]{0.28\linewidth} 
    \centering
    \parbox{2.5cm}{\centering \scriptsize \textbf{Ground}\\\textbf{Truth}} \par\vspace{3pt}
    \includegraphics[width=\linewidth]{#1/gt.png}
  \end{minipage}%
  \hfill % Push grid to right
  % --- Right Block: Labels + 4 Columns of Methods ---
  \begin{minipage}[c]{0.71\linewidth}
    \centering
    \tiny % Use tiny text to fit method names
    % 5 columns: 1 label column + 4 method columns
    \begin{tabular}{@{}c@{\hspace{2pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{\hspace{1pt}}c@{}}
      % --- Header Row ---
      % Parbox width increased to 2.5cm to match larger image width
      &
      \parbox{2.5cm}{\centering W/O Higher\\Order Dynamics} & 
      \parbox{2.5cm}{\centering W/O $P(\alpha \mid \theta, C, T)$} & 
      \parbox{2.5cm}{\centering W/O\\Stochasticity} & 
      \parbox{2.5cm}{\centering \textbf{GraphiTS (Ours)}} \\[5pt]
      
      % --- Row 1: Crop A ---
      \vclbl{#4} &
      \vcimg{#1/no_higher_#2_a.png} &
      \vcimg{#1/no_likeli_#2_a.png} &
      \vcimg{#1/deterministic_#2_a.png} &
      \vcimg{#1/graphits_#2_a.png} \\
      \noalign{\vspace{1pt}} % Force exact 1pt vertical gap

      % --- Row 2: Crop B ---
      \vclbl{#5} &
      \vcimg{#1/no_higher_#3_a.png} &
      \vcimg{#1/no_likeli_#3_a.png} &
      \vcimg{#1/deterministic_#3_a.png} &
      \vcimg{#1/graphits_#3_a.png} \\
      
    \end{tabular}
  \end{minipage}
}
